Vulnerability anti-patterns in Solidity: Increasing smart contracts security by reducing false alarms

Turing completeness has made Ethereum smart contracts attractive to blockchain developers and attackers alike. To increase code security, many tools can now spot most known vulnerabilities$-$at the cost of production efficiency. Recent studies show false-positive ratios over 99% in state-of-the-art technologies: this makes them impractical for use in industry and have raised questions on the direction of academic research. In this work we show how integrating and extending current analyses is not only feasible, but also a next logical step in smart-contract security. We propose light-weight static checks on the morphology and dynamics of Solidity code, stemming from a developer-centric notion of vulnerability, that we use to verify the output of other tools, flag potential false alarms, and suggest verifications. Besides technical details we implemented an open-source prototype. For three top-10 vulnerabilities it flags 324 warnings of other tools as false-positives, in 60 verified de-duplicated smart contracts selected from the blockchain by the presence of true (and false) vulnerabilities. This amounts to a 92%- to 100%-reduction in the number of false-positives for these vulnerabilities.

==> tables/Related_Works.tex <==
\begin{tabularx}{\linewidth}{|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
\hline
\rowcolor[HTML]{C0C0C0}
\textbf{Paper Title} & \textbf{Common Points} & \textbf{Differences (what we add)} \\
\hline

Redetect: Reentrancy vulnerability detection in smart contracts with high accuracy \cite{Yu.2021} &
\multirow{2}{=}{They study the limitations of current methods and tools that attempt to flag reentrancy vulnerabilities in smart contracts. These works propose code patterns attributable to false positives, and \cite{Yu.2021} introduces ReDetect, a symbolic-execution tool for reentrancy vulnerabilities discovery, that mitigates false positives via filters tailored to recognize previously identified patterns.} &
\multirow{2}{=}{Our work covers two vulnerabilities besides reentrancy, with the (met) expectation to identify patterns common between them, and the extra requirement of fast-checking times as per \Cref{RQ:tools_enhancement}.} \\
\cline{1-1}

Turn the Rudder: A beacon of reentrancy detection for smart contracts on Ethereum \cite{ZZS+23} & & \\ 
\hline

sCompile: Critical Path Identification and Analysis for Smart Contracts \cite{Chang.2018} &
Introduce the sCompile tool, which analyses the control-flow graph (CFG) of a smart contract to find ``critical paths'', i.e. paths which involve monetary transaction (sic), and prioritize those which potentially violate important properties. The goal is to reduce the number of false positives, which they demonstrate via comparisons against the Maian tool (see \Cref{sec:tools}). &
The ultimate goal coincides with ours, which is to reduce the number of false positives. The approach used in this paper though focuses on patterns that can be associated with a high degree of confidence with true positives, while our focus is on patterns that can be associated with false negatives. \\
\hline

An empirical evaluation of the effectiveness of smart contract verification tools \cite{Dias.2021} &
\multirow{3}{=}{They assess the efficacy of tools that analyse vulnerabilities in Solidity smart contracts, reporting a prevalence of false positives. While the evaluation in \cite{Dias.2021} is used to learn how the assessed tools can complement each other, \cite{HLSL23,PL21} are concerned with the proportion of vulnerable-flagged contracts that are effectively exploited in the Ethereum blockchain, which can be as low 1\% for certain vulnerability types. In particular, \cite[Fig.~5]{HLSL23} identifies code patterns that can be associated with the generation of false alarms. These works are thus in close connection to our \Cref{RQ:tools_available,RQ:tools_quality}.} &
\multirow{3}{=}{We extend by implementing a prototypical tool that we use to obtain empirical data on the effectiveness (and efficiency) of these extended checks.} \\
\cline{1-1}

Why smart contracts reported as vulnerable were not exploited? \cite{HLSL23} & & \\
\cline{1-1}

Smart contract vulnerabilities: Vulnerable does not imply exploited \cite{PL21} & & \\
\hline

Empirical review of automated analysis tools on 47,587 Ethereum smart contracts \cite{DFAC20} &
\multirow{2}{=}{Propose benchmarking approaches for smart contracts security tools. In particular, \cite{DFAC20} introduces the SmartBugs execution framework, while \cite{GP20} puts forth SolidiFI, a bug-injection approach that allows to produce artificial vulnerable contracts. Both papers use what has been proposed to evaluate SotA analysis tools on large datasets.} &
\multirow{2}{=}{We also assess 3rd party software---in a much more modest scale---but as an intermediate goal, used to identify false-positive patterns as in \cite{HLSL23}, which we use in experiments that demonstrate the practical feasibility of our findings. In addition, our tests are conducted on a dataset of contracts, really deployed on the ethereum blockchain, analyzed manually.} \\
\cline{1-1}

How effective are smart contract analysis tools? Evaluating smart contract static analysis tools using bug injection \cite{GP20} & & \\
\hline
\end{tabularx}

%%	In this subsection, we shall conduct a comparative examination of pertinent academic literature akin to our study, with particular emphasis on delineating their points of differentiation.
%%	\begin{itemize}
%%	\item   \cite{ZZS+23},\cite{Yu.2021}: 
%%	        Both of these studies focus on Reentrancy-type vulnerabilities, aiming to show the limitations, especially in terms of producing false positives, of SotA tools designed for analyzing Solidity-based smart contracts. In both articles, a number of patterns attributable to these false positives are identified. \cite{Yu.2021} differs from \cite{ZZS+23} primarily in its proposal of an innovative tool, ReDetect, founded on symbolic execution, which endeavors to identify Reentrancy-type vulnerabilities while mitigating the issue of false positives through the incorporation of filters tailored to recognized previously identified patterns. 
%%	        Notably, our research diverges from these studies in terms of the range of vulnerabilities examined, which extends beyond Reentrancy, also covering Unchecked Call Return Value and Timestamp Dependence. In addition, compared to \cite{Yu.2021}, the results of our proposed tool, Detecti, have been compared with more SotA tools in order to get a broader view.
%%	\item   \cite{Chang.2018}:
%%	        The authors underscore the prevalence of false positives generated by contemporary tools available for Solidity code analysis. Subsequently, the authors introduce sCompile, a tool predicated on identifying precarious pathways within contracts. sCompile underwent testing on approximately 200 contracts, with its outcomes juxtaposed against those of Maian, another tool for Solidity vulnerability detection, revealing a markedly reduced incidence of false positives. In contrast to the primary focus of this article on identifying potentially hazardous patterns, our research delves into the intricacies of false positive generation, shedding light on nuances often overlooked in vulnerability detection.
%%	\item   \cite{Dias.2021},\cite{HLSL23}:
%%	        In both of these research works, the primary aim is to assess the efficacy of widely used tools for the analysis of Solidity smart contracts within the context of a vulnerability detection. The investigation yielded notable findings, particularly an observed prevalence of false positives in both instances. The study presented in \cite{Dias.2021} further delves into an evaluation of the strengths and weaknesses inherent in each tool, ultimately identifying a form of complementarity among them. Conversely, the examination in \cite{HLSL23} focuses on delineating patterns commonly associated with the generation of these erroneous alerts. Our research, akin to the aforementioned studies, evaluates prominent tools but expands beyond conventional performance metrics. Our analysis uniquely encompasses the identification of patterns specific to individual vulnerabilities, in contrast to the generic applicability of false positive patterns discussed in \cite{HLSL23}. In addition, unlike both of these articles, we introduce a prototype aimed at addressing this persistent challenge, thereby offering a novel contribution to the field.
%%	\item   \cite{DFAC20},\cite{GP20}:
%%	        The core theme in both articles revolves around streamlining and automating the assessment of analysis tools for smart contracts. In \cite{DFAC20}, the introduction of SmartBugs, an execution framework, takes center stage, while \cite{GP20} puts forth SolidiFI, a systematic and automated approach involving the intentional injection of bugs, or code defects, into potential locations within a smart contract to deliberately induce targeted security vulnerabilities. Both studies then proceed to conduct tests using datasets comprising thousands of contracts, revealing a significant issue with the generation of numerous false positives. In \cite{GP20}, the presence of some false negatives is also acknowledged, prompting an analysis to identify commonly associated patterns. Our research aligns with these endeavors in terms of the testing phase of various tools and the subsequent analysis of results. However, our focus diverges as we concentrate on three specific vulnerabilities and primarily identify patterns linked to false positives. Additionally, our contribution extends to the proposal of a tool designed to address and overcome these identified limitations.
%%	\item   \cite{PL21}:
%%	        In this paper, the authors aim to ascertain the extent to which contracts identified as vulnerable were genuinely exploited through attacks. Their methodology involved employing six different tools on a dataset comprising approximately 821,000 contracts, identifying those labeled as vulnerable, and subsequently determining if they were targeted in attacks via transaction analysis. The findings reveal that only a minute fraction, less than 1\%, of the contracts flagged as vulnerable were actually subject to attacks, presumably through the detected vulnerabilities. This outcome is attributed to the presumption of a substantial number of false positives, however, unlike our article, this assumption is not corroborated through a thorough analysis of the contracts and identification of underlying causes.
%%	\end{itemize}


==> tables/badges.tex <==
\begin{tabularx}{\textwidth}{|X|X|X|X|X|X|}
\hline
\textbf{Badge Name} & \textbf{Badge Icon} & \textbf{Availability Criteria} & \textbf{Installation Criteria} & \textbf{Usage INPUT criteria} & \textbf{Usage OUTPUT criteria} \\
\hline
Artifact Available & \raisebox{-.5\height}{\includegraphics[width=0.8\linewidth]{figures/artifacts_available.jpg}} & Level = 1 & any & any & any \\
\hline
Artifact Evaluated-Functional & \raisebox{-.5\height}{\includegraphics[width=0.8\linewidth]{figures/artifacts_evaluated_functional.jpg}} & Level <= 2 & Level <= 2 & Level <= 2 & Level <= 2 \\
\hline
Artifact Evaluated-Reusable & \raisebox{-.5\height}{\includegraphics[width=0.8\linewidth]{figures/artifacts_evaluated_reusable.jpg}} & Level <= 2 & Level = 1 & Level = 1 & Level = 1 \\
\hline
\end{tabularx}

==> tables/criteria.tex <==
\renewcommand{\arraystretch}{0.2}
\begin{tabularx}{\textwidth}{|>{\centering\arraybackslash}m{0.5cm}|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
\hline
& \textbf{Availability Criteria (C1)} & \textbf{Installation Criteria (C2)} & \textbf{Usage INPUT criteria (C3)} & \textbf{Usage OUTPUT criteria (C4)} \\ 
\hline
\rotatebox{90}{\textbf{Level 1}} & \cellcolor[HTML]{D9EAD3}A tool is proposed and it is publicly accessible to all & \cellcolor[HTML]{D9EAD3}Installation is possible using the instructions given in the repository/artifact and is very simple (\textless{}=5 commands). & \cellcolor[HTML]{D9EAD3}Command to launch the analysis provided, explaining each parameter in detail. It succeeds on the first try & \cellcolor[HTML]{D9EAD3}The output returned is very clear and tidy, allowing the user to understand it from the first use of the tool \\ 
\hline
\rotatebox{90}{\textbf{Level 2}} & \cellcolor[HTML]{F4CCCC}A tool is proposed but is not made available or is only made available upon direct request to the authors & \cellcolor[HTML]{D9EAD3}Installation is possible by following the instructions in the repository/artifact but it is rather long (\textgreater{}5 instructions) & \cellcolor[HTML]{D9EAD3}Command to launch analysis provided, but details are missing (ex.: parameter explanation). It takes some trial and error before it succeeds. & \cellcolor[HTML]{D9EAD3}The returned output is rather complex and/or messy, risking generating confusion, but the information deriving from the analysis is nevertheless provided \\ 
\hline
\rotatebox{90}{\textbf{Level 3}} & \cellcolor[HTML]{F4CCCC}What is proposed is only at a theoretical level (approach, technique, or similar things) & \cellcolor[HTML]{D9EAD3}Multiple installation methods are proposed in the repository/artifact, but only a few (1/2) actually work & \cellcolor[HTML]{F4CCCC}Command not provided or only an example is provided, totally lacking in explanation so that it is possible to generalize & \cellcolor[HTML]{F4CCCC}The output shows operational errors and it is not possible to obtain the results of the analysis, or in any case they can only be obtained partially \\ 
\hline
\rotatebox{90}{\textbf{Level 4}} & / & \cellcolor[HTML]{F4CCCC}It is not possible to correctly install the tool only with the instructions given in the repository/artifact, you must carry out external searches for solutions. & / & / \\ 
\hline
\rotatebox{90}{\textbf{Level 5}} & / & \cellcolor[HTML]{F4CCCC}You can't install even by searching on the web (incompatibility of libraries, correct environment not indicated, etc.) & / & / \\ 
\hline
\end{tabularx}

==> tables/info_REE.tex <==
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c }
\hline
\multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}}                                 & \_50Win                                                                                                                                                                                                                                                                                                                                                                                                          & Dice                                                                                                  & HeroUp                                                                                                                                                                                     & RugPull                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & JAY                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & BNBBrokers                                                                                                                                                                                                                                                                                                                                                           & Token                                                                                                                                                                                                                                                                                                                                                                          & CrystalDeposit                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & Zethroll                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & IMDEXDexchange                                                                                                                                                                                                                                                                                                                                                                                                      & KiOS                                                                                                                                                                                                                                                                                                               & Sale                                                                                                                                                                                                         & Issuer                                                                                                                                                                                                                                                                                                                                                                                                                                                            & contractDeployer                                                                                                                                                                                                                                                                                      & BitizenCarOperator                                                                                                                                                                                                                                                                                                                                                                                                                                     & BatchTransferWallet                                                                                                                                                                                                                                                                                             & FairWin                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & PERSONAL\_BANK                                                                                                                                                 & EthToSmthSwaps                                                                                                                                                                                                                                                                                                                                    & Convert                                                                       \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Address}                        & 0x79aD73567e7f9A5b4a2D28264F78aff9D971CF14                                                                                                                                                                                                                                                                                                                                                                       & 0xB3d8f628BDa4592a0e35A693e9Ae8C413879929B                                                            & 0x56C945f90c9Cd1aAfbcaC78936f569e5Fd2438BF                                                                                                                                                 & 0xf7A190028d34e16483B58e7a925701Da29F274c4                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & 0xf2919D1D80Aff2940274014bef534f7791906FF2                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & 0x2C67f86D91BA3cA559c6d2825d9dbD00C5A90e4B                                                                                                                                                                                                                                                                                                             & 0x003FfEFeFBC4a6F34a62A3cA7b7937a880065BCB                                                                                                                                                                                                                                                                                                                                     & 0x00676065A7854163c6a4D5F474496514D03E31C4                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & 0x0096dc2246FC3627Cc2bF87a3B0d2e0f87B58589                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & 0x00c315AC9Ff89bb6aFa7524CD159f0a9766e8c89                                                                                                                                                                                                                                                                                                                                                                          & 0x00F634a0bB03416816F8829928eF7D776F798414                                                                                                                                                                                                                                                                         & 0x00FA44D91D7541D16DD18A48dd6A011de5E887DF                                                                                                                                                                   & 0x012bc399c3E8B75A506c9ff2B7ad413641F33102                                                                                                                                                                                                                                                                                                                                                                                                                        & 0x019e41A2ACDffAFC0303e840fbD7934234e68F45                                                                                                                                                                                                                                                            & 0x01de9415D1aE14AB755186bEa22923AFe2934d82                                                                                                                                                                                                                                                                                                                                                                                                             & 0x01e0F57c42bf976676eA1dAa1B04d69ABa6bDAF3                                                                                                                                                                                                                                                                      & 0x01EaCc3Ae59eE7fBBC191d63E8e1ccfdAc11628C                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & 0x01F8c4E3Fa3EdEb29e514cba738D87CE8C091d3f                                                                                                                     & 0x025DcE2d39a46296766DB7CAC8c322E8f59CD5D9                                                                                                                                                                                                                                                                                                        & 0x0297FdbCb9c2023Bc05ad44c9F6E69B0aE6261cE                                    \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Solidity Version}               & \textgreater=0.6.8                                                                                                                                                                                                                                                                                                                                                                                              & \textgreater=0.6.0 \textless0.8.0                                                                        & 0.4.24                                                                                                                                                                                     & 0.6.6                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            & 0.8.0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   & 0.6.10                                                                                                                                                                                                                                                                                                                                                               & 0.4.16                                                                                                                                                                                                                                                                                                                                                                         & 0.4.25                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & 0.4.23                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & 0.4.23                                                                                                                                                                                                                                                                                                                                                                                                              & 0.4.25                                                                                                                                                                                                                                                                                                             & 0.4.13                                                                                                                                                                                                       & /                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & 0.4.21                                                                                                                                                                                                                                                                                                & 0.4.24                                                                                                                                                                                                                                                                                                                                                                                                                                                 & 0.4.24                                                                                                                                                                                                                                                                                                          & 0.4.24                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & 0.4.19                                                                                                                                                         & 0.4.23                                                                                                                                                                                                                                                                                                                                            & 0.4.21                                                                        \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Functions}                      & send / cancelBet / takeBet                                                                                                                                                                                                                                                                                                                                                                                       & userWithdraw / adminWithdraw / emergencyWithdraw                                                      & reclaimToken / upgrade                                                                                                                                                                     & withdraw / tokenFallback / buy / transferToContract / transfer / constructor                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & buyNFTs / buyJay / sell / buyJayNoNFT / buyJayWithERC721 / buyERC721 / updateFees / buyJayWithERC1155 / buyERC1155 / getLatestPrice                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & setCommissionWallet / invest / withdraw                                                                                                                                                                                                                                                                                                                              & airDropToken / withdrawToken / approveAndCall                                                                                                                                                                                                                                                                                                                                  & setContractsMiniGame / setMiningWarInterface / setEngineerInterface / startGame / startRound / share / getEngineerPrizePool / constructor / endRound / withdrawReward                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & constructor / ownerTransferZTH / ownerSetBankroll / ownerkill / \_finishBet / finishBet / \_playerRollDice / tokenFallback                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & IMDEXdepositToken / IMDEXwithdrawToken / IMDEXadminWithdraw                                                                                                                                                                                                                                                                                                                                                         & pay / buy / getBalance                                                                                                                                                                                                                                                                                             & buyTokens /\&nbsp;\&nbsp;fallback                                                                                                                                                                            & issue / recoverTokens / tokensToBeReturned                                                                                                                                                                                                                                                                                                                                                                                                   & deployToken / deployCrowdsale / multiSender                                                                                                                                                                                                                                                           & getOwnerCars / getCarInfo / createCar / createCarByOperator                                                                                                                                                                                                                                                                                                                                                                                            & batchTransfer/ withdraw / balanceOfContract                                                                                                                                                                                                                                                                     & invest / remedy / userWithDraw / countShareAndRecommendedAward / countRecommend / execute                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & collect / deposit                                                                                                                                              & withdraw / close / refund / abort                                                                                                                                                                                                                                                                                                                 & getNewToken                                                                   \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}TPs}                            & 2                                                                                                                                                                                                                                                                                                                                                                                                                & 0                                                                                                     & 0                                                                                                                                                                                          & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       & 0                                                                                                                                                                                                                                                                                                                                                                    & 0                                                                                                                                                                                                                                                                                                                                                                              & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & 0                                                                                                                                                                                                                                                                                                                                                                                                                   & 0                                                                                                                                                                                                                                                                                                                  & 0                                                                                                                                                                                                            & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & 0                                                                                                                                                                                                                                                                                                     & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                      & 0                                                                                                                                                                                                                                                                                                               & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & 1                                                                                                                                                              & 0                                                                                                                                                                                                                                                                                                                                                 & 0                                                                             \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}FPs}                            & 1                                                                                                                                                                                                                                                                                                                                                                                                                & 3                                                                                                     & 2                                                                                                                                                                                          & 6                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & 10                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & 3                                                                                                                                                                                                                                                                                                                                                                    & 3                                                                                                                                                                                                                                                                                                                                                                              & 10                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & 8                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              & 3                                                                                                                                                                                                                                                                                                                                                                                                                   & 3                                                                                                                                                                                                                                                                                                                  & 2                                                                                                                                                                                                            & 3                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & 3                                                                                                                                                                                                                                                                                                     & 4                                                                                                                                                                                                                                                                                                                                                                                                                                                      & 3                                                                                                                                                                                                                                                                                                               & 6                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & 1                                                                                                                                                              & 4                                                                                                                                                                                                                                                                                                                                                 & 1                                                                             \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}justification of vulnerability} & send is private / cancelBet is actually a TP beacuse send is called before the removeBet function / even takeBet is a TP even if it is a bit more difficult to exploit, you will need to accept a bvet with another addr always controlled by you, this way you will have every time to send a value=bet.value, but each reentrancy iteration one of the two accounts controlled by you will receive 2Xbet.value & userWithdraw, adminWithdraw, and emergencyWithdraw are callable only by owner because of the modifier & reclaimToken is a FP beacuse there is no state change after it (last instruction) / upgrade is a FP beacuse all the external functions are called from an address not controllable by user & withdraw is a FP beacuse there is no state change after externall call (there is only emission of event) / tokenFallback is a FP beacuse there is a if condition requiring the msg.sender to be equal to hardcoded address + call called on DEV, which is an hardcoded address corresponding to the owner of contract + external function withdraw is called on PiZZa which is hardcoded / buy is a FP because the address of which the function is executed is PiZZa, which is hardcode / transferToContract is a FP because there is no state change after externall call + private visibility / transfer is a FP beacuse there is still not state change after externall call & buyNFTs is a FP beacuse call is called on dev, which is the hardcoded address of owner / buyJay is a FP beacuse call is called on dev, which is the hardcoded address of owner / sell is a FP because there is no state change after externall call (just event emission) / buyJayNoNFT is a FP beacuse call is called on dev, which is the hardcoded address of owner / buyJayWithERC721 is a FP beacuse it is internal + no state change after externall call + transfer is from msg.sender to contract / buyERC721 is a FP beacuse it is internal + no state change after externall call / updateFees is a FP because the adr on which function is called (priceFeed) is not controllable by user / buyJayWithERC1155 is a FP beacuse it is internal + no state change after it / buyERC1155 is a FP beacuse it is internal + no state change after it / getLatestPrice is a FP beacuse there is no state change after externall call + hard-coded address & setCommissionWallet is a FP beacuse there is the require checking that caller is owner / invest is a FP because the call is called on commissionWallet, which is an hardcoded address / withdraw is a FP because the 1st call is called on commissionWallet, which is an hardcoded address + the 2nd call is not followed by a state change (only emission of event) & airDropToken is a FP beacuse there is no state change after it (only emission of event) + onlyOwner modifier / withdrawToken is a FP beacuse there is no state change after external call (last instruction) + modifier allowing only owner to call this / approveAndCall is a FP beacuse there is no state change after external call (last instrcution) & setContractsMiniGame is a FP beacuse the modifier is allowing only administrator to call the function / setMiningWarInterface is a FP beacuse the modifier is allowing only administrator to call the function / setEngineerInterface is a FP beacuse the modifier is allowing only administrator to call the function / startGame is a FP beacuse the modifier is allowing only administrator to call the function + the address on which the function is called is hard-coded / startRound is a FP beacuse the modifier is allowing only administrator to call the function + the address on which function is called is hard-coded / share is a FP because the address on which function is called is hard-coded / getEngineerPrizePool is a FP because the address on which function is called is hard-coded + there is no state change after it / constructor is a FP for its nature, called only once by SC creator + it would be a FP anyway beacuse of the modifier of the functions called / account\_info\_rotate\_tine is a FP beacuse the called function is a FP beacuse the function is called on an hard-coded address / withdrawReward is a FP -\textgreater see motivation of endRound() & constructor is a FP beacuse its nature (called only once by owner when contract created) + no state change after call of external function / ownerTransferZTH is a FP beacuse the modfier is allowing only owner to call this function + no state change after external function (only event emission) + hard-coded address/ ownerSetBankroll is a FP beacuse the modfier is allowing only owner to call this function + hard-coded address / ownerkill\&nbsp;\&nbsp;is a FP beacuse the modfier is allowing only owner to call this function + hard-coded address / dumpdivs is a FP beacuse the address from which is called the function is hard-coded + no state change after it / \_finishBet is a FP beacuse it is private + hard-coded address + no state change after externall call / finishBet is a FP -\textgreater see motivation \_finishBet / \_playerRollDice is a FP -\textgreater it is private + see motivation \_finishBet / tokenFallback is a FP -\textgreater see motivation \_playerRollDice & IMDEXdepositToken is a FP beacuse the external function is transferring tokens from user to this contract + no state change after it (only event emission) / IMDEXwithdrawToken is a FP because there is no state change after it (only event emission) -\textgreater the state change is correctly before /  IMDEXadminWithdraw is a FP beacuse the modifier is allowing only admin to call this & pay is a FP beacuse the modifier is allowing only admin to call it + no state change after it (only event emission) / buy is a Fp because there is no state change after it (only event emission) / getBalance is a FP because there is no state change after externall call + it is internal & buyTokens is a FP beacuse the address from which function is called is hard-coded + no state change after function (only event emission) / fallback is a FP beacuse it is literally only calling buyTokens() & issue is a FP beacuse the modifier is allowing onbly the owner to call it + the address from which function is called is hard-coded / recoverTokens is a FP beacuse the modifier is allowing onbly the owner to call it / recoverEthers is a FP beacuse the modifier is allowing onbly the owner to call it + address hard-coded / tokensToBeReturned is a FP because there is no state change after it + function not transferring anything & deployToken and deployCrowdsale are FPs because there is no state change after external function (only event emission) + hard-coded address / multiSender is a FP beacuse the first external function is called on hard-coded address and all 3 external functions are not followed by a state change & getOwnerCars\&nbsp;\&nbsp;and getCarInfo are FP beacuse the address from which function is called is hardcoded + there is no state change after it / createCar is a FP because the address from which function is called is hardcoded + there is no state change after it (only event emission) / createCarByOperator is a FP because the address from which function is called is hardcoded + there is no state change after it (only event emission) & batchTransfer is a FP beacuse there is no state change after the two external functions / withdraw is a FP beacuse there is no state change after the two external functions (only emission of event) + modifier onlyOwner / balanceOfContract is a FP beacuse there is no state change after external function & invest is a FP because all the external functions are called on the util address which is hardcoded / remedy is a FP because all the external functions are called on the util address which is hardcoded / userWithDraw is a FP because all the external functions are called on the util address which is hardcoded / countShareAndRecommendedAward is a FP because all the external functions are called on the util address which is hardcoded + onlyOwner modifier / countRecommend is a FP because all the external functions are called on the util address which is hardcoded / execute is a FP because all the external functions are called on the util address which is hardcoded + private but it is called by public function & collect is a TP -\textgreater user can drain all contract balance before updating his balance / deposit is a FP because the state is not changed after externall call & withdraw is a FP because the address from which the function is called is hard-coded / close is a FP because the address from which the function is called is hard-coded / refund is a FP because the address from which the function is called is hard-coded / abort is a FP because the address from which the function is called is hard-coded & getNewToken is a FP because the function is called from an hard-coded address \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Notes}                          &                                                                                                                                                                                                                                                                                                                                                                                                                  & For Slither had to use solidity version 0.7.6                                                         &                                                                                                                                                                                            &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         &                                                                                                                                                                                                                                                                                                                                                                      & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                                                                                                                                                                                                     &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &                                                                                                                                                                                                                                                                                                                                                                                                                     &                                                                                                                                                                                                                                                                                                                    &                                                                                                                                                                                                              & (for Mythril had to add solidity version to contract, set to 0.4.24)                                                                                                                                                                                                                                                                                                                                                                                              &                                                                                                                                                                                                                                                                                                       &                                                                                                                                                                                                                                                                                                                                                                                                                                                        &                                                                                                                                                                                                                                                                                                                 &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            &                                                                                                                                                                &                                                                                                                                                                                                                                                                                                                                                   &                                                                               \\ \hline
\end{tabular}

==> tables/info_TD.tex <==
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c }
\hline
\multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}}                                    & BCFVault                                                                                                                                                        & DMINT                                                                                                                                                                                                                                               & FifteenPlus                                                                                                                                                                                                                                                                                                                                                                                                                     & FtvTimelockFactory                                                                                                                                                                          & HeartBoutPreICO                                                                                                                                                                                                                                                                                                                                                                                                                      & MultisigWallet                                                                                                                                                                 & EthCapsule                                                                                                                                                                                                                                                                                                                                                                                                                                                                & GIFT\_ENVELOPE                                                                                                                                                                                                   & RockCoin                                                                                                                                                                                                                                                                       & StupidCrowdsale                                                                                              & DepoX                                                                                                              & C\_banK                                                                                                                                                                                                                              & BDTToken                                                                                                                                                                                                                                                                                                                                                                                      & RobocallsTokenSale                                                                                                                                                                                                                                  & MOIRAICO                                                                                                                                                                                                                                                                                                                                                                                           & OpenLongevityPresale                                                                                                                                                                                                                                 & TimeBankToken                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & hodlEthereum                                                                                        & BountyBG                                                                                                                                                                                                                                                                                                                                                                                   & IdGameCoin                                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Address}                           & 0x001b22d44e1b8edf01c1bccd08bb99e2e6198092                                                                                                                      & 0x51c6a6Ef1352578Ff01B078313E6779B88BDcb1E                                                                                                                                                                                                          & 0xcfd2047eb61412e9b8de511dc2087e07003829ee                                                                                                                                                                                                                                                                                                                                                                                      & 0xd0080a841a8c5d2b6cd4bc640cdad7846de14dbf                                                                                                                                                  & 0x0d62442a4b931ac1243997d96bfe37fef4fb03e7                                                                                                                                                                                                                                                                                                                                                                                           & 0x7199C3fBc0832e8798d2514eEAa88f0CE597698D                                                                                                                                     & 0x5274a2293DBE075a82D41E873Bb927403a9dCE46                                                                                                                                                                                                                                                                                                                                                                                                                                & 0xbF5fb038c28df2B8821988DA78C3EBDBf7Aa5Ac7                                                                                                                                                                       & 0xdfBd6A960a55bCfCf59d5925351E05a51498BCeF                                                                                                                                                                                                                                     & 0x002842529757eab873cce9c251087e1b993f9200                                                                   & 0x021e5e6aB3eFE5eB0c060B4C4C523C7470787ef5                                                                         & 0x02242d41C54F261a85ac8E8efa7046a3Dfd53113                                                                                                                                                                                           & 0x033030FEeBd93E3178487c35A9c8cA80874353C9                                                                                                                                                                                                                                                                                                                                                    & 0x0d4D61D5B3e4F46c54D175935881d0faA356Fca1                                                                                                                                                                                                          & 0x0f5ee401De162Cd163b6Ff46318Eef2727dBb9fc                                                                                                                                                                                                                                                                                                                                                         & 0x179A303C1fdFF0fFBdA6a68B384787621B78ee84                                                                                                                                                                                                           & 0x18Ce0b9FeDCeB66e9fB7783BbdDB4565232a9c22                                                                                                                                                                                                                                                                                                                                                                                                                                                            & 0x1BB28e79f2482df6bf60efc7a33365703bCF1536                                                          & 0x1e200A9af1aB6A0d74cD44C489Bf65744BC7d961                                                                                                                                                                                                                                                                                                                                                 & 0x209132061047FF4D2ad395691005D3266e48b673                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Solidity Version}                  & 0.4.24                                                                                                                                                          & 0.4.11                                                                                                                                                                                                                                              & 0.4.24                                                                                                                                                                                                                                                                                                                                                                                                                          & 0.4.11                                                                                                                                                                                      & 0.4.18                                                                                                                                                                                                                                                                                                                                                                                                                               & 0.4.11                                                                                                                                                                         & 0.4.11                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & 0.4.19                                                                                                                                                                                                           & 0.4.11                                                                                                                                                                                                                                                                         & 0.4.18                                                                                                       & 0.4.25                                                                                                             & 0.4.25                                                                                                                                                                                                                               & 0.4.23                                                                                                                                                                                                                                                                                                                                                                                        & 0.4.24                                                                                                                                                                                                                                              & 0.4.11                                                                                                                                                                                                                                                                                                                                                                                             & 0.4.10                                                                                                                                                                                                                                               & 0.4.11                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & 0.4.11                                                                                              & 0.4.14                                                                                                                                                                                                                                                                                                                                                                                     & 0.4.19                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Instructions containing timestamp} & \begin{tabular}[c]{@{}c@{}}1. joined{[}msg.sender{]} = block.timestamp;\\ 2. uint256 minutesCount = now.sub(joined{[}\_address{]}).div(1 minutes);\end{tabular} & 1. randomNumber += block.timestamp + uint(msg.sender);                                                                                                                                                                                              & \begin{tabular}[c]{@{}c@{}}1. if((now-prtime{[}owner{]}) \textgreater= 86400)\{\\ 2. prtime{[}owner{]} = now;\\ 3. uint256 paymentAmount = balance{[}msg.sender{]}*rate{[}msg.sender{]}/1000*(now-timestamp{[}msg.sender{]})/86400;\\ 4. timestamp{[}msg.sender{]} = now;\end{tabular}                                                                                                                                                 & 1. require(releaseTimes{[}\_holder{]} \textless now, "release time is not met yet");                                                                                                        & \begin{tabular}[c]{@{}c@{}}1. require(\_startTime \textgreater= now);\\ 2. bool withinPeriod = now \textgreater= startTime \&\& now \textless= endTime;\\ 3. return now \textgreater endTime;\end{tabular}                                                                                                                                                                                                                    & 1. return now / 1 days;                                                                                                                                                        & \begin{tabular}[c]{@{}c@{}}1. require(unlockTime \textless= block.timestamp + maxDuration);\\ 2. if (unlockTime \textless block.timestamp + minDuration) \{\\ 3. unlockTime = SafeMath.add(block.timestamp, minDuration);\\ 4. lockTime: block.timestamp,\\ 5. require(capsule.unlockTime \textless= block.timestamp);\\ 6. capsule.withdrawnTime = block.timestamp;\end{tabular}                                                                                         & \begin{tabular}[c]{@{}c@{}}1. if(hashPass == keccak256(pass) \&\& now\textgreater giftTime)\\ 2. if(msg.sender==reciver \&\& now\textgreater giftTime)\\ 3. giftTime = now;\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. saleTimeStart = now;\\ 2. if (!preSale \&\& saleTimeStart + 5 weeks \textless now \&\& !burned) \{\end{tabular}                                                                                                                      & 1. require(now \textgreater= startTime \&\& now \textless= endTime);                            & 1. if (msg.sender==Owner \&\& now\textgreater=open) \{                                                & \begin{tabular}[c]{@{}c@{}}1. acc.unlockTime = \_unlockTime\textgreater now?\_unlockTime:now;\\ 2. if( acc.balance\textgreater=MinSum \&\& acc.balance\textgreater=\_am \&\& now\textgreater acc.unlockTime)\\ 3. LastMsg.Time = now;\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. return ICOstarttime \textless now \&\& now \textless ICOendtime;\\ 2. if(now \textgreater= 1533128400 \&\& now \textless 1534337940)\{\\ 3. else if(now \textgreater= 1534338000 \&\& now \textless 1535547600)\{\\ 4. else if(now \textgreater 1536152400 \&\& now \textless 1542204000)\{\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. bonusEnds = now + 8 weeks;\\ 2. endDate = now + 8 weeks;\\ 3. startDate = now;\\ 4. require(now \textgreater= startDate \&\& now \textless= endDate);\\ 5. if (now \textless= bonusEnds) \{\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. uint startTime = now;\\ 2. else if(state == State.Preico \&\& now \textless (startTime + 1 days)) \{\\ 3. if(now \textless ICOdeadline \&\& state!=State.Successful)\{\\ 4. if(now \textgreater preICODeadline \&\& state==State.Preico)\{\\ 5. else if(now \textgreater ICOdeadline \&\& state!=State.Successful) \{\\ 6. completedAt = now;\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. require(now \textless presaleFinishTime);\\ 2. if (now \textgreater presaleFinishTime) \{\\ 3. t = presaleFinishTime - now;\\ 4. require(now \textgreater= presaleFinishTime || collectedUSD == totalLimitUSD);\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. return(tokenBalances{[}\_tokenAddress{]}{[}\_holder{]}.timeToWithdraw, tokenBalances{[}\_tokenAddress{]}{[}\_holder{]}.numTokens, block.timestamp);\\ 2. require(\_amount \textgreater 0 \&\& \_time \textgreater block.timestamp \&\& \_time \textless block.timestamp + 157680000);\\ 3. require(tokenBalances{[}\_token{]}{[}msg.sender{]}.timeToWithdraw \textless block.timestamp \&\& tokens \textgreater 0);\end{tabular} & 1. require (block.timestamp \textgreater partyTime \&\& hodlers{[}msg.sender{]} \textgreater 0);          & \begin{tabular}[c]{@{}c@{}}1. require(\\ ...\\ bounty.startTime + bountyDuration \textgreater block.timestamp \&\&\\ ...\\ );\\ 2. bounty.endTime = block.timestamp;\\ 3. bounty.endTime = block.timestamp;\\ 4. bounty.startTime = block.timestamp;\\ 5. require(\\ ... \&\&\\ bounty.startTime + bountyDuration \textless block.timestamp\\ );\end{tabular} & \begin{tabular}[c]{@{}c@{}}1. startPreIco = now;\\ 2. if (now \textless= bonusEnds) \{\\ 3. require (now \textgreater= startPreIco \&\& now \textless= bonusEnds);\\ 4. require (now \textgreater= startIco \& now\textless= endIco);\\ 5. if (now \textless= bonusEnds) \{\end{tabular} \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}TPs}                               & 2                                                                                                                                                               & 1                                                                                                                                                                                                                                                   & 2                                                                                                                                                                                                                                                                                                                                                                                                                               & 0                                                                                                                                                                                           & 0                                                                                                                                                                                                                                                                                                                                                                                                                                    & 0                                                                                                                                                                              & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & 0                                                                                                                                                                                                                & 0                                                                                                                                                                                                                                                                              & 0                                                                                                            & 0                                                                                                                  & 0                                                                                                                                                                                                                                    & 0                                                                                                                                                                                                                                                                                                                                                                                             & 0                                                                                                                                                                                                                                                   & 0                                                                                                                                                                                                                                                                                                                                                                                                  & 0                                                                                                                                                                                                                                                    & 0                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & 0                                                                                                   & 0                                                                                                                                                                                                                                                                                                                                                                                          & 0                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}FPs}                               & 0                                                                                                                                                               & 0                                                                                                                                                                                                                                                   & 2                                                                                                                                                                                                                                                                                                                                                                                                                               & 1                                                                                                                                                                                           & 4                                                                                                                                                                                                                                                                                                                                                                                                                                    & 1                                                                                                                                                                              & 6                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & 3                                                                                                                                                                                                                & 2                                                                                                                                                                                                                                                                              & 2                                                                                                            & 1                                                                                                                  & 4                                                                                                                                                                                                                                    & 8                                                                                                                                                                                                                                                                                                                                                                                             & 6                                                                                                                                                                                                                                                   & 6                                                                                                                                                                                                                                                                                                                                                                                                  & 4                                                                                                                                                                                                                                                    & 4                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & 1                                                                                                   & 5                                                                                                                                                                                                                                                                                                                                                                                          & 7                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Justification of Vulnerability}    & TPs: Both uses of timestamp (block.timestamp and now) are problematic because the defined variables are then indirectly used to determine the user balance      & TP: The timestamp is used indirectly to define a variable (reward) which is then added to the balance of the user. There is not an ETH transfer taking as amount a variable influenced by timestamp but I still would consider this a true positive & \begin{tabular}[c]{@{}c@{}}Fps: The first two uses of now are confined to the use inside condition regulating an IF statement which is checking for certain value to be larger (checking time interval). \\ TPs: While the last two uses of the timestamp (definition of paymentAmount e timestamp{[}msg.sender{]} variables) are influencing the amount of crypto to be transferred through transfer instruction"\end{tabular} & FP: The only use of timestamp is inside a require condition checking for it to be larger than another value (checking that a specific time has been passed), and consequently not dangerous & \begin{tabular}[c]{@{}c@{}}Fps: The first require check if \_startTime has passed. Return value (including withinPeriod) of validPurchase function is just used inside require condition to check that tokens are buyed only during valid period. hasEnded function is never called inside contract, just information for user.\\ Overall the use of timestamp is limited to check time intervals"\end{tabular} & FP: The today function is called only within if conditions that test time intervals or otherwise to define the lastDay variable whose use is limited to such conditions anyway & FPs: it is possible to see that all if and require conditions that directly contain the timestamp verify time intervals. As for the variables defined with the timestamp: the use of unlockTime is limited to the same conditions. locktime is not used anywhere, only information. capsule.withdrawnTime is used in a require statement and compared to 0, but again results in a false positive since it is not possible to manipulate the block timestamp to reset it. & FPs: The two if conditions use the timestamp only to verify that it is greater than the value contained in the giftTime variable, whose purpose is solely this comparison. (check time interval)                 & FPs: The condition uses the timestamp to verify that it is within the valid period for sales. To do this, the timestamp is compared with the variable saleTimeStart, which contains the timestamp of the time of the start of sales and is exclusively used in this condition. & FP: Again the require is intended to verify that the sale of tokens occurs only during the valid time period & FP: the only use of timestamp is inside if condition checking to be later than the time saved in the open variable & FPs: The if condition compares the timestamp with the value of the acc.unlockTime variable (its only use), then checks that the unlock interval has arrived. LastMsg.Time is never used, only information.                           & FPs: All three if conditions use timestamps to verify time intervals. The ICOactive function is uniquely called in a require statement, again with the intent of verifying that the contract execution is in the valid period                                                                                                                                                                 & FPs: The if and require conditions that directly contain the timestamp are used to verify time intervals. Variables defined using the timestamp are exclusively used in the preceding conditions.                                                   & FPs: All if conditions that directly use the timestamp are aimed at checking time intervals. The variable startTime is used to define other variables (preICODeadline and ICOdeadline), but all are used exclusively within the previous if conditions to verify time intervals. The completedAt variable is never used, only information.                                                         & FPs: All if and require conditions that directly use the timestamp are aimed at checking time intervals. The function timeToFinishPresale is returning t variable but it is not called anywhere, only user info                                      & FPs: Both require conditions that directly use the timestamp are aimed at checking time intervals. The function getInfo is not called anywhere, only user info                                                                                                                                                                                                                                                                                                                                        & FPs: The only require condition that directly use the timestamp is aimed at checking time interval. & FPs: Both require conditions that directly use the timestamp are aimed at checking time intervals. bounty.endTime variable is used only inside a return statement for user information purposes. bounty.startTime is only used inside previous seen require conditions, always for checking time intervals                                                                                 & FPs: All if and require conditions that directly use the timestamp are aimed at checking time intervals. startPreIco variable is exclusively used in one of these conditions, again for the purpose of verifying a time interval.                                                                                     \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Notes}                             &                                                                                                                                                                 &                                                                                                                                                                                                                                                     &                                                                                                                                                                                                                                                                                                                                                                                                                                 & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                  &                                                                                                                                                                                                                                                                                                                                                                                                                                      &                                                                                                                                                                                &                                                                                                                                                                                                                                                                                                                                                                                                                                                                           &                                                                                                                                                                                                                  &                                                                                                                                                                                                                                                                                &                                                                                                              &                                                                                                                    &                                                                                                                                                                                                                                      &                                                                                                                                                                                                                                                                                                                                                                                               &                                                                                                                                                                                                                                                     & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                                                                                                                                                                                                                         & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                                                                           &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       &                                                                                                     & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                                                                                                                                                                                                                 & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                                                                                                                                            \\ \hline
\end{tabular}

==> tables/info_UEC.tex <==
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c 
>{\columncolor[HTML]{FFFFFF}}c 
>{\columncolor[HTML]{EFEFEF}}c 
>{\columncolor[HTML]{C0C0C0}}c }
\hline
\multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}}                                 & EasyInvest25                                                                                          & EasyInvest10                                                                                                                                                                                                                                                                                       & Escrow                                                                                                                                                                                                                                                               & EtherprisesLLC                                                                                                                                                           & Game                                                                                                                                                                                                                                                                                & MyNewBank                                                                                                                                                                                                                       & Getether                                                                                                                                                                                                                                                                                   & PonziScheme                                                                                                                                                             & WithdrawDAO                                                                                           & EncryptedToken                                                                                                                                                                                                                                      & EDProxy                                                                                                                                                                                                              & SmartBlockchainPro                                                                                                                                                                                                                                                                    & JJCOIN                                                                                                                                                                                                                                                                                                                                                            & TokenBank                                                                                                                                                                                                                                                                                                                     & airdrop                                                                  & Ninja                                                                                     & BitProCoinX                                                                                                         & EtherDice                                                                                                                                                                                                                                                                                                                                                                                                                                   & BuyRoseCoin                                                                                                      & WealthRedistributionProject                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Address}                        & 0x06faa4d8157ba45baf2da5e7d02384225948d54f                                                            & 0x0744a686c17480b457a4fbb743195bf2815ca2b8                                                                                                                                                                                                                                                         & 0x073e957bc883693f15ecb14bfced3e8ffc8654c5                                                                                                                                                                                                                           & 0x0d47d4aea9da60953fd4ae5c47d2165977c7fbea                                                                                                                               & 0xc741bc7fa502ddcf2d5cc9e2c70f0ee7090cfd0d                                                                                                                                                                                                                                          & 0x52c2d09acf0ef12c487ae0c20a92d4f9a4abbfd1                                                                                                                                                                                      & 0x0b19DC8df2F75AE40C10c871Ab95e3bFBE98fB5c                                                                                                                                                                                                                                                 & 0xc58492b3b14f658adff566c988029308505f81b5                                                                                                                              & 0xc58d783e39aabe61a4bce8d4b5e7264e67c92c27                                                            & 0x48966E7591ed845E0177E4D2442643e874531b5d                                                                                                                                                                                                          & 0x02F66A7d5657Ee67be39349988aa1F944206eAd3                                                                                                                                                                           & 0x0513CE8013F27A47a0088fFAaC94fbb0fe6309d8                                                                                                                                                                                                                                            & 0x26987c0b7712bf1DF35b3781a3E96e793091D95b                                                                                                                                                                                                                                                                                                                        & 0x39CFD754c85023648Bf003beA2Dd498c5612AbFA                                                                                                                                                                                                                                                                                    & 0x4051334adc52057aCa763453820cb0e045076eF3                               & 0x40EAC8F2702758275AbBbda2881708f82c417a7F                                                & 0x50f7c95b7e82eA5E0953DE8c7EaD20A9DD289Ec2                                                                          & 0x5138e7b13E56Ac9b15654cC2824a28e5355Af4B4                                                                                                                                                                                                                                                                                                                                                                                                  & 0x0614e57bBc71cd0B15217152D4B07AF5E717D4eF                                                                       & 0x3325439082FF8ba7371DFdAa1AF297bBfcAc21b2                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Solidity Version}               & 0.4.24                                                                                                & 0.4.24                                                                                                                                                                                                                                                                                             & /                                                                                                                                                                                                                                                                    & 0.4.9                                                                                                                                                                    & 0.4.3                                                                                                                                                                                                                                                                               & 0.4.17                                                                                                                                                                                                                          & 0.4.25                                                                                                                                                                                                                                                                                     & 0.4.11                                                                                                                                                                  & /                                                                                                     & 0.4.25                                                                                                                                                                                                                                              & 0.4.4                                                                                                                                                                                                                & 0.4.25                                                                                                                                                                                                                                                                                & 0.4.2                                                                                                                                                                                                                                                                                                                                                             & 0.4.18                                                                                                                                                                                                                                                                                                                        & 0.4.24                                                                   & 0.4.20                                                                                    & 0.4.16                                                                                                              & 0.4.25                                                                                                                                                                                                                                                                                                                                                                                                                                      & 0.4.11                                                                                                           & /                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}TPs}                            & 0                                                                                                     & 1                                                                                                                                                                                                                                                                                                  & 0                                                                                                                                                                                                                                                                    & 0                                                                                                                                                                        & 0                                                                                                                                                                                                                                                                                   & 0                                                                                                                                                                                                                               & 1                                                                                                                                                                                                                                                                                          & 0                                                                                                                                                                       & 0                                                                                                     & 1                                                                                                                                                                                                                                                   & 0                                                                                                                                                                                                                    & 1                                                                                                                                                                                                                                                                                     & 0                                                                                                                                                                                                                                                                                                                                                                 & 0                                                                                                                                                                                                                                                                                                                             & 0                                                                        & 0                                                                                         & 0                                                                                                                   & 0                                                                                                                                                                                                                                                                                                                                                                                                                                           & 0                                                                                                                & 1                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}FPs}                            & 1                                                                                                     & 1                                                                                                                                                                                                                                                                                                  & 2                                                                                                                                                                                                                                                                    & 1                                                                                                                                                                        & 2                                                                                                                                                                                                                                                                                   & 1                                                                                                                                                                                                                               & 1                                                                                                                                                                                                                                                                                          & 1                                                                                                                                                                       & 1                                                                                                     & 0                                                                                                                                                                                                                                                   & 1                                                                                                                                                                                                                    & 1                                                                                                                                                                                                                                                                                     & 2                                                                                                                                                                                                                                                                                                                                                                 & 2                                                                                                                                                                                                                                                                                                                             & 1                                                                        & 1                                                                                         & 1                                                                                                                   & 1                                                                                                                                                                                                                                                                                                                                                                                                                                           & 1                                                                                                                & 1                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Justification of Vulnerability} & 1 kashout.send (EasyInvest25.fallback): FP -\textgreater address on which is called is the msg.sender & \begin{tabular}[c]{@{}c@{}}1 owner.send (EasyInvest10.fallback): TP -\textgreater the fail of the transaction to the owner could mean more crypto to be transferred to the attacker\\ 2 kashout.send (EasyInvest10.fallback): FP -\textgreater address on which is called is the msg.sender\end{tabular} & \begin{tabular}[c]{@{}c@{}}1 seller.send (Escrow.finalize):FP -\textgreater condition requiring msg.sender to be equal to hardcoded address + no state modification after send (last instruction)\\ 2 buyer.send (Escrow.refund): FP -\textgreater same as first send\end{tabular} & 1 generalManager.send (EtherprisesLLC.withdraw): FP -\textgreater modifier checking msg.sender equal to hardcoded address + no state change after send & \begin{tabular}[c]{@{}c@{}}1 founder.send (Game.open): FP -\textgreater modifier checkFounder is allowig the function to be called only by founder\\ 2 user.send (Game.withdraw): FP -\textgreater same as 1st send + there is no state change after send (last instruction)\end{tabular} & 1 msg.sender.send (MyNewBank.withdraw): FP -\textgreater modifier onlyowner is allowig the function to be called only by owner + the address on which send is called is msg.sender + no state modification after it (last instruction) & \begin{tabular}[c]{@{}c@{}}1 owner.send (Getether.fallback): TP -\textgreater the fail of the transaction to the owner could mean more crypto to be transferred to the attacker\\ 2 kashout.send (Getether.fallback): FP -\textgreater address on which is called is the msg.sender\end{tabular} & 1 lastDepositor.send (PonziScheme.fallback): FP -\textgreater there is not a real possible advantage for the attacker, despite not even falling in any of the FPs patterns & 1 trustee.send (WithdrawDAO.trusteeWithdraw): FP -\textgreater no state change after send (last instruction) & 1 owner.send (EncryptedToken.fallback): TP -\textgreater The attacker can reduce the balanceOf{[}owner{]} even if the owner has not actually received the send crypto (the attacker has to still pay / no other ways for owner to withdraw ETH balance) & 1 \_callee.delegatecall (EDProxy.dtrade): FP -\textgreater no state change after it (last instruction), even considering when called by testcall function                                                               & \begin{tabular}[c]{@{}c@{}}1 sender.send (SmartBlockchainPro.fallback): FP -\textgreater send is called on msg.sender\\ 2 marketingAddr.send (SmartBlockchainPro.fallback): TP -\textgreater fail of crypto transfer to owner can mean more balance to withdraw in future for attacker\end{tabular} & \begin{tabular}[c]{@{}c@{}}1 msg.sender.send (JJCOIN.constructor): FP -\textgreater send is called on msg.sender + no state change after it (last instruction) + it is in the constructor\\ 2 owner.send (JJCOIN.collectExcess): FP -\textgreater modifier is allowing only the owner to call the function + no state change after send (last instruction)\end{tabular} & \begin{tabular}[c]{@{}c@{}}1 token.call (Ownable.WithdrawToken): FP -\textgreater modifier is allowing only the owner to call the function + no state change after call (last instruction)\\ 2 \_addr.call.value (Ownable.WithdrawToHolder): FP -\textgreater modifier is allowing only the owner to call the function\end{tabular} & 1 caddress.call (airdrop.transfer): FP -\textgreater no state change after call & 1 hodl.call (Ninja.fallback): FP -\textgreater no state change after call (last instruction) & 1 owner.send (BitProCoinX.withdraw): FP -\textgreater modifier onlyOwner + no state change after it (last instruction) & 1 \_receiver.send (EtherDice.send): FP -\textgreater the flow considered is starting with fallback function, which is calling the createBet function, which is calling sendOwner, which is calling the send function.If the send instruction fails the attacker can place the bets without the fee being correctly sent to owner, but this last one can still withdraw it from balance through withdraw function & 1 owner.send (RoseCoin.withdraw): FP -\textgreater modifier onlyOwner + no state change after it (last instruction) & \begin{tabular}[c]{@{}c@{}}1 msg.sender.send (WealthRedistributionProject.enter): FP -\textgreater send is called on msg.sender + no state change after it (last instruction)\\ 2 benefactor{[}k{]}.etherAddress.send (WealthRedistributionProject.enter): TP -\textgreater a failed send to another address means that such user will lose his/her payment for that transaction and will have no way to recover it\end{tabular} \\ \hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}Notes}                          &                                                                                                       &                                                                                                                                                                                                                                                                                                    &                                                                                                                                                                                                                                                                      &                                                                                                                                                                          &                                                                                                                                                                                                                                                                                     &                                                                                                                                                                                                                                 &                                                                                                                                                                                                                                                                                            &                                                                                                                                                                         &                                                                                                       &                                                                                                                                                                                                                                                     & \begin{tabular}[c]{@{}c@{}}(for Mythril had to change the solidity version to 0.4.24)\\ Had to modify the code beacuse there was an error -\&amp;gt; removing round brackets around second delegatecall\end{tabular} &                                                                                                                                                                                                                                                                                       & (for Mythril had to change the solidity version to 0.4.24)                                                                                                                                                                                                                                                                                                        &                                                                                                                                                                                                                                                                                                                               &                                                                          & (for Mythril had to change the solidity version to 0.4.24)                                &                                                                                                                     &                                                                                                                                                                                                                                                                                                                                                                                                                                             &                                                                                                                  & (for Mythril had to add the solidity version to 0.4.24)                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\end{tabular}

==> tables/results_REE.tex <==
\colcolortablepreamble
\begin{tabular}{%
	>{~}L{10em}@{}   % contract name
	>{~\columncolor{shade4}}c@{~~~}c@{\quad}  % Ground Truth
	>{~~\columncolor{shade3}}c@{~~~}c@{~~~~}  % Slither
	>{~~\columncolor{shade3}}c@{~~~}c@{~~~~}  % Mythril
	>{~~\columncolor{shade3}}c@{~~~}c@{~~}     % Remix
}
\toprule
	& \multicolumn{2}{>{~}c@{~~~~}}{\bfseries Ground truth}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Slither}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Mythril}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Remix}
\\
\arrayrulecolor{black!50}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){2-3}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){4-5}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){6-7}
\cmidrule[.8pt](l{.5pt}r{2.5pt}){8-9}
\arrayrulecolor{black}
%\rotatebox{90}{$\looparrowleft$}\;\raisebox{3pt}{Smart contract}
Smart contract
	& ~~$\mathsf{P+N}$~~  % all relevant instructions...
	& $\mathsf{P}$        % ...of which are vulnerable
	& \FP,\FN\, & \TP,\TN  % Slither
	& \FP,\FN\, & \TP,\TN  % Mythril
	& \FP,\FN\, & \TP,\TN  % Remix
\\\midrule
%
\code{\_50Win}
	& 1 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{1}  % Mythril
	& \twores{1}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{Decore}
	& 3 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{2}  % Slither
	& \twores{1}{0}~ & \twores{0}{2}  % Mythril
	& \twores{1}{0}~ & \twores{0}{2}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{Dice}
	& 3 & 0  % Ground Truth
	& \twores{3}{0}~ & \twores{0}{0}  % Slither
	& \twores{3}{0}~ & \twores{0}{0}  % Mythril
	& \twores{3}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{MagicLamp}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{2}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{PumpETH}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{2}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{QORE}
	& 3 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{2}  % Slither
	& \twores{1}{0}~ & \twores{0}{2}  % Mythril
	& \twores{2}{0}~ & \twores{0}{1}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{RugPull}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{2}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{JAY}
	& 4 & 0  % Ground Truth
	& \twores{4}{0}~ & \twores{0}{0}  % Slither
	& \twores{1}{0}~ & \twores{0}{3}  % Mythril
	& \twores{4}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{BNBBrokers}
	& 3 & 0  % Ground Truth
	& \twores{3}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{3}  % Mythril
	& \twores{3}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}          {TP}        {TN}
\\
\code{XCORE}
	& 3 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{2}  % Slither
	& \twores{1}{0}~ & \twores{0}{2}  % Mythril
	& \twores{2}{0}~ & \twores{0}{1}  % Remix
	%       {FP}{FN}         {TP}{TN}
\\\midrule
\raggedleft\textbf{Total:}\hspace*{.5em}
	& $\mathbf{26}$ & $\mathbf{0}$  % Ground Truth
	& $\mathbf{\twores{20}{0}~}$ & $\mathbf{\twores{0}{6}}$  % Slither
	& $\mathbf{\twores{7}{0}~}$  & $\mathbf{\twores{0}{19}}$  % Mythril
	& $\mathbf{\twores{22}{0}~}$ & $\mathbf{\twores{0}{4}}$  % Remix
	%                 {FP}{FN}                    {TP}{TN}
\\[-.5ex]
\rowcolor{white}
\multicolumn{3}{>{~}r@{~~}}{\itshape\Detecti:}
	& \tworesit{20}{0}~ & \tworesit{0}{6}  % Slither
	& \tworesit{7}{0}~  & \tworesit{0}{19}  % Mythril
	& \tworesit{22}{0}~ & \tworesit{0}{4}  % Remix
	%       {FP}{FN}          {TP}{TN}
\\\bottomrule
\end{tabular}


==> tables/results_TD.tex <==
\colcolortablepreamble
\begin{tabular}{%
	>{~}L{10em}@{}   % contract name
	>{~\columncolor{shade4}}c@{~~~}c@{\quad}  % Ground Truth
	>{~~\columncolor{shade3}}c@{~~~}c@{~~~~}  % Slither
	>{~~\columncolor{shade3}}c@{~~~}c@{~~~~}  % Mythril
	>{~~\columncolor{shade3}}c@{~~~}c@{~~}     % Remix
}
\toprule
	& \multicolumn{2}{>{~}c@{~~~~}}{\bfseries Ground truth}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Slither}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Mythril}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Remix}
\\
\arrayrulecolor{black!50}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){2-3}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){4-5}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){6-7}
\cmidrule[.8pt](l{.5pt}r{2.5pt}){8-9}
\arrayrulecolor{black}
%\rotatebox{90}{$\looparrowleft$}\;\raisebox{3pt}{Smart contract}
Smart contract
	& ~~$\mathsf{P+N}$~~  % all relevant instructions...
	& $\mathsf{P}$        % ...of which are vulnerable
	& \FP,\FN\, & \TP,\TN  % Slither
	& \FP,\FN\, & \TP,\TN  % Mythril
	& \FP,\FN\, & \TP,\TN  % Remix
\\\midrule
%
\code{BCFVault}
	& 2 & 2  % Ground Truth
	& \twores{0}{0}~         & \twores{2\miss{1}}{0}  % Slither
	& \twores{0}{2\miss{1}}~ & \twores{0}        {0}  % Mythril
	& \twores{0}{0}~         & \twores{2\miss{1}}{0}  % Remix
	%       {FP}{FN}                  {TP}{TN}
\\
\code{DMINT}
	& 1 & 1  % Ground Truth
	& \twores{0}{0}~         & \twores{1\miss{1}}{0}  % Slither
	& \twores{0}{1\miss{1}}~ & \twores{0}        {0}  % Mythril
	& \twores{0}{0}~         & \twores{1\miss{1}}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{FifteenPlus}
	& 4 & 4  % Ground Truth
	& \twores{0}{0}~         & \twores{4\miss{2}}{0}  % Slither
	& \twores{0}{2\miss{1}}~ & \twores{2\miss{1}}{0}  % Mythril
	& \twores{0}{0}~         & \twores{4\miss{2}}{0}  % Remix
	%       {FP}{FN}                  {TP}       {TN}
\\
\code{FtvTimelockFactory }
	& 1 & 1  % Ground Truth
	& \twores{0}{0}~ & \twores{1}{0}  % Slither
	%& \multicolumn{2}{>{\columncolor{black!60}}c@{~~~}}{\color{white}\code{ERROR}}  % Mythril
	& \multicolumn{2}{>{}c@{~~~}}{\framebox[7em]{\smaller\code{ERROR}}}  % Mythril
	& \twores{0}{0}~ & \twores{1}{0}  % Remix
	%       {FP}{FN}         {TP}{TN}
\\
\code{HeartBoutPreICO }
	& 3 & 2  % Ground Truth
	& \twores{1\miss{1}}{0}~         & \twores{2\miss{2}}{0}  % Slither
	& \twores{1\miss{1}}{1\miss{1}}~ & \twores{1\miss{1}}{0}  % Mythril
	& \twores{1\miss{1}}{0}~         & \twores{2\miss{2}}{0}  % Remix
	%       {FP}{FN}                          {TP}       {TN}
\\
\code{MultisigWallet}
	& 1 & 0  % Ground Truth
	& \twores{1\miss{1}}{0}~ & \twores{0}        {0}  % Slither
	& \twores{0}        {0}~ & \twores{1\miss{1}}{0}  % Mythril
	& \twores{1\miss{1}}{0}~ & \twores{0}        {0}  % Remix
	%       {FP}       {FN}           {TP}       {TN}
\\
\code{EthCapsule}
	& 6 & 3  % Ground Truth
	& \twores{2}{0}~         & \twores{3\miss{2}}{1}  % Slither
	& \twores{1}{1\miss{1}}~ & \twores{2\miss{1}}{2}  % Mythril
	& \twores{3}{0}~         & \twores{3\miss{2}}{0}  % Remix
	%       {FP}{FN}                  {TP}       {TN}
\\
\code{GIFT\_ENVELOPE}
	& 3 & 3  % Ground Truth
	& \twores{0}{0}~ & \twores{3\miss{1}}{0}  % Slither
	& \multicolumn{2}{>{}c@{~~~}}{\framebox[7em]{\smaller\code{ERROR}}}  % Mythril
	& \twores{0}{0}~ & \twores{3\miss{1}}{0}  % Remix
	%       {FP}{FN}          {TP}       {TN}
\\
\code{RockCoin}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{2}{0}~ & \twores{0}{0}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}         {TP}{TN}
\\
\code{StupidCrowdsale}
	& 1 & 1  % Ground Truth
	& \twores{0}{0}~ & \twores{1}{0}  % Slither
	& \twores{0}{0}~ & \twores{1}{0}  % Mythril
	& \twores{0}{0}~ & \twores{1}{0}  % Remix
	%       {FP}{FN}         {TP}{TN}
\\\midrule
\raggedleft\textbf{Total:}\hspace*{.5em}
	& $\mathbf{24}$ & $\mathbf{17}$  % Ground Truth
	& $\mathbf{\twores{6}{0}~}$ & $\mathbf{\twores{17}{1}}$  % Slither
	& $\mathbf{\twores{4}{7}~}$ & $\mathbf{\twores{7}{2}}$  % Mythril
	& $\mathbf{\twores{7}{0}~}$ & $\mathbf{\twores{17}{0}}$  % Remix
	%                 {FP}{FN}                    {TP}{TN}
\\[-.5ex]
\rowcolor{white}
\multicolumn{3}{>{~}r@{~~}}{\itshape\Detecti:}
	& \tworesit{4}{0}~ & \tworesit{7}{1}  % Slither
	& \tworesit{3}{1}~ & \tworesit{3}{2}  % Mythril
	& \tworesit{5}{0}~ & \tworesit{7}{0}  % Remix
	%       {FP}{FN}         {TP}{TN}
\\\bottomrule
\end{tabular}


==> tables/results_UEC.tex <==
\colcolortablepreamble
\begin{tabular}{%
	>{~}L{10em}@{}   % contract name
	>{~\columncolor{shade4}}c@{~~~}c@{\quad}  % Ground Truth
	>{~~\columncolor{shade3}}c@{~~~}c@{~~~~}  % Slither
	>{~~\columncolor{shade3}}c@{~~~}c@{~~~~}  % Mythril
	>{~~\columncolor{shade3}}c@{~~~}c@{~~}     % Remix
}
\toprule
	& \multicolumn{2}{>{~}c@{~~~~}}{\bfseries Ground truth}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Slither}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Mythril}
	& \multicolumn{2}{>{~~}c@{~~~}}{\bfseries Remix}
\\
\arrayrulecolor{black!50}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){2-3}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){4-5}
\cmidrule[.8pt](l{.5pt}r{5.5pt}){6-7}
\cmidrule[.8pt](l{.5pt}r{2.5pt}){8-9}
\arrayrulecolor{black}
%\rotatebox{90}{$\looparrowleft$}\;\raisebox{3pt}{Smart contract}
Smart contract
	& ~~$\mathsf{P+N}$~~  % all relevant instructions...
	& $\mathsf{P}$        % ...of which are vulnerable
	& \FP,\FN\, & \TP,\TN  % Slither
	& \FP,\FN\, & \TP,\TN  % Mythril
	& \FP,\FN\, & \TP,\TN  % Remix
\\\midrule
%
\code{EasyInvest25}
	& 1 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{1}  % Mythril
	& \twores{1}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{EasyInvest10}
	& 2 & 1  % Ground Truth
	& \twores{1}{0}~ & \twores{1}{0}  % Slither
	& \twores{0}{0}~ & \twores{1}{1}  % Mythril
	& \twores{1}{0}~ & \twores{1}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{Escrow}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{1}{0}~ & \twores{0}{1}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{EtherGarden}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{2}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{EtherprisesLLC}
	& 1 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{0}  % Slither
	& \twores{1}{0}~ & \twores{0}{0}  % Mythril
	& \twores{1}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{Game}
	& 2 & 0  % Ground Truth
	& \twores{2}{0}~ & \twores{0}{0}  % Slither
	& \twores{2}{0}~ & \twores{0}{0}  % Mythril
	& \twores{2}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{MyNewBank}
	& 1 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{0}  % Slither
	& \twores{1}{0}~ & \twores{0}{0}  % Mythril
	& \twores{1}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{GetEther}
	& 2 & 1  % Ground Truth
	& \twores{1}{0}~ & \twores{1}{0}  % Slither
	& \twores{0}{0}~ & \twores{1}{1}  % Mythril
	& \twores{1}{0}~ & \twores{1}{0}  % Remix
	%       {FP}{FN}        {TP}{TN}
\\
\code{PonziScheme}
	& 1 & 1  % Ground Truth
	& \twores{0}{0}~ & \twores{1\miss{1}}{0}  % Slither
	& \twores{0}{0}~ & \twores{1\miss{1}}{0}  % Mythril
	& \twores{0}{0}~ & \twores{1\miss{1}}{0}  % Remix
	%       {FP}{FN}          {TP}       {TN}
\\
\code{WithdrawDAO}
	& 1 & 0  % Ground Truth
	& \twores{1}{0}~ & \twores{0}{0}  % Slither
	& \twores{0}{0}~ & \twores{0}{1}  % Mythril
	& \twores{1}{0}~ & \twores{0}{0}  % Remix
	%       {FP}{FN}         {TP}{TN}
\\\midrule
\raggedleft\textbf{Total:}\hspace*{.5em}
	& $\mathbf{15}$ & $\mathbf{3}$  % Ground Truth
	& $\mathbf{\twores{12}{0}~}$ & $\mathbf{\tworesit{3}{0}}$  % Slither
	& $\mathbf{\twores{5}{0}~}$  & $\mathbf{\tworesit{3}{7}}$  % Mythril
	& $\mathbf{\twores{12}{0}~}$ & $\mathbf{\tworesit{3}{0}}$  % Remix
	%                 {FP}{FN}                    {TP}{TN}
\\[-.5ex]
\rowcolor{white}
\multicolumn{3}{>{~}r@{~~}}{\itshape\Detecti:}
	& \tworesit{12}{0}~ & \tworesit{2}{0}  % Slither
	& \tworesit{5}{0}~  & \tworesit{2}{7}  % Mythril
	& \tworesit{12}{0}~ & \tworesit{2}{0}  % Remix
	%       {FP}{FN}          {TP}{TN}
\\\bottomrule
\end{tabular}


==> tables/tools-eligibility.tex <==
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}c| c|cccc|c}
\hline
Name           & \begin{tabular}[c]{@{}c@{}}Vuln. Detected\\ (among 3 considered)\end{tabular} & C1                        & C2                        & C3                        & C4                        & \textbf{Eligible}           \\ \hline
Oyente         & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}3 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Mythril        & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}3 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Osiris         & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}3 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Securify       & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}4 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Maian          & -                                                                             & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Zeus           & URV / REE                                                                     & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Slither        & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}YES \\ \hline
SmartCheck     & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Remix          & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}- & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Manticore      & Not Indicated                                                                 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Sereum         & REE                                                                           & \cellcolor[HTML]{FFCCC9}3 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Vandal         & URV / REE                                                                     & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
ContractFuzzer & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
MadMax         & -                                                                             & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
ReGuard        & REE                                                                           & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
EasyFlow       & -                                                                             & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Vultron        & URV / REE                                                                     & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
VeriSmart      & Not Indicated                                                                 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Harvey         & URV / REE                                                                     & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
sFuzz          & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{FFCCC9}3 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Seraph         & REE                                                                           & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Echidna        & -                                                                             & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
SmartShield    & URV / REE                                                                     & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
ContractWard   & URV / REE / TD                                                                & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
ConFuzzius     & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}3 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Solscan        & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
eThor          & REE                                                                           & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{FFCCC9}3 & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Ethlint        & URV / TD                                                                      & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Medusa         & -                                                                             & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
Halmos         & Not Indicated                                                                 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}3 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
S-Gram         & Not Indicated                                                                 & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Gasper         & -                                                                             & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
WANA           & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}3 & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
SmartScopy     & URV / REE / TD                                                                & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
ExGen          & REE                                                                           & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
SoliDetector   & URV / REE / TD                                                                & \cellcolor[HTML]{FFCCC9}2 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
Horstify       & URV / REE / TD                                                                & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{FFCCC9}5 & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}- & \cellcolor[HTML]{FFCCC9}NO  \\ \hline
AChecker       & -                                                                             & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}YES \\ \hline
EtherSolve     & Ree                                                                           & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}1 & \cellcolor[HTML]{9AFF99}2 & \cellcolor[HTML]{9AFF99}YES \\ \hline
\end{tabular}

==> tables/tools.tex <==
\def\ALIGN{\centering}%~\\}
\def\TOOL#1{\parbox[t]{3em}{\ALIGN\protect{#1}\\[.5ex]\protect{\cite{#1}}}}
\def\NOPE{\parbox[t]{2em}{\ALIGN No}}
\def\YEP{\parbox[t]{2em}{\ALIGN\bfseries Yes}}
%
\begin{tabular}{>{\!\!}c@{~~~}L{.36\linewidth}@{~~}c@{~~}L{.36\linewidth}}
\toprule
	\bfseries Tool
	& \bfseries Description
	& \bfseries \!\!\!Match
	& \bfseries Main reason
\\\midrule\arrayrulecolor{black!50}
%
\TOOL{Oyente}
	& Symbolic execution. Parses source- and byte-code. Vulnerabilities: reentrancy, timestamp dependence, transaction-order dependence, unchecked external call.
	& \NOPE
	& Installation and usability: following instruction failed to deploy a consistently working tool (last GitHub update 4 years ago, causing library dependency issues).
%%	It is a tool based on symbolic execution, so it can statically reason about a program path-by-path. The tool covers four different types of vulnerabilities, the three that our work is focused on plus "Transaction-Ordering Dependence". %This tool can receive as input both source code in Solidity and compiled code in the form of EVM bytecode. What made us discard this tool for our tests were the innumerable difficulties encountered during its installation, despite the fact that we followed the instructions provided by the authors. In addition, performing a contract analysis returns a variety of warnings indicating conflicts in the versions of the libraries used.
\\\midrule[.3pt]
%
\TOOL{Osiris}
	& Symbolic execution and taint analysis (leverages Oyente). Vulnerabilities: integer under- \& overflow. % Parses source- and byte-code
	& \NOPE
	& Vulnerabilities covered do not match our interest set.
%%	It is a framework that combines symbolic execution and taint analysis, in order to accurately identify integer bugs in Ethereum smart contracts. It should also be pointed out that this tool was implemented on top of Oyente's symbolic execution engine. %The tool analyzes EVM bytecode, but can also receive as input Solidity code that is compiled internally before analysis.  In this case what led us to discard this tool was the narrowness of the vulnerabilities considered, which were limited to integer bugs. It is also a type of vulnerability that we did not address.
\\\midrule[.3pt]
%
\TOOL{Mythril}
	& Symbolic execution, \acronym{smt} solving, and taint analysis. Vulnerabilities: 16 in total (see \cite{Mythril}) + severity rating.\!
	& \YEP
	& Swift installation through Docker image, and vulnerabilities match our interest set.
%%	It is a security analysis tool for EVM bytecode, which uses a combination of symbolic execution, SMT solving and taint analysis. Mythril can detect a total of 16 different types of vulnerabilities, including the three covered by our prototype, and rates them with severity ratings to indicate the level of danger. The choice to use this tool as a benchmark is due to the ease of installation through the Docker image and the variety of vulnerabilities detected.
\\\midrule[.3pt]
%
\TOOL{Securify}
	& Symbolic execution with \acronym{dsl} for vulnerability pattern-matching, and security properties definition. Vulnerabilities: 37 in total (see \cite{Securify}).
	& \NOPE
	& v1.0 is deprecated, and v2.0 (was easy to install but) works for Solidity v5.8.0 and above, which reduces severely the test set of smart contracts.
%%	It is good to specify that what we considered is the second version of the tool, Securify 2.0; the first version is now deprecated. This tool analysis consists of two steps. First, it symbolically analyzes the contract’s dependency graph to extract precise semantic information from the code. Then, it checks compliance and violation patterns that capture sufficient conditions for proving if a property holds or not. To enable extensibility, all patterns are specified in a designated domain-specific language. This tool allows detection of a total of as many as 37 vulnerabilities, including the three covered in our prototype. The ease of installation and use, coupled with the broad coverage of vulnerability types make Securify extremely interesting, except that it can only analyze contracts written with versions of Solidity equal to or newer than 5.8.0, making it not applicable to most of the smart contracts we collected, which is why it was discarded.
\\\midrule[.3pt]
%
\TOOL{Maian}
	& Specification and validation of trace properties via symbolic analysis. Vulnerabilities: trace-related, e.g.\ funds locking and leaking.
	& \NOPE
	& Vulnerabilities covered do not match our interest set.
%%	It is the first tool for specifying and reasoning about trace properties, which employs inter-procedural symbolic analysis and concrete validator for exhibiting real exploits.  This tool focuses attention on three example properties of such trace vulnerabilities: finding contracts that either lock funds indefinitely, leak them carelessly to arbitrary users, or can be killed by anyone. As you can see, none of these vulnerabilities coincides with those we chose for our work, thus being a determining factor in our choice not to take this tool as a benchmark.
\\\midrule[.3pt]
%
\TOOL{Zeus}
	& Formal verification (model checking), with wizard to match source code to a  XACML template. Vulnerabilities: 5 types, including reentrancy and unchecked external call.
	& \NOPE
	& Installation and usability: following instruction failed to deploy a consistently working tool.
%%	It is a practical framework for automatic formal verification of smart contracts using abstract interpretation and symbolic model checking. It takes as input the smart contracts written in high-level languages and leverages user assistance to help generate the correctness and/or fairness criteria in a XACMLstyled template. The tool can detect 5 types of vulnerabilities, including "Unchecked Call Return Value" (for which, however, it is limited to the send function) and "Reentrancy", but does not include the third vulnerability we cover, "Timestamp Dependence". This incomplete coverage of the vulnerabilities of our interest, coupled with the difficulties encountered during installation due to the numerous requirements, are the reasons that led us to exclude this tool from our work.
\\\midrule[.3pt]
%
\TOOL{Slither}
	& Static checker and taint analysis, via the SlithIR intermediate representation. Vulnerabilities: 93 (see \cite{Slither}).
	& \YEP
	& Easy installation and use, and vulnerabilities math our interest set.
%%	It is a static analysis framework designed to provide rich information about Ethereum smart contracts. Slither allows for the application of commonly used program analysis techniques like dataflow and taint tracking. SlithIR is the hybrid intermediate representation used in Slither to represent Solidity code. Ninety-three different detectors are implemented in the tool and used to detect as many types of vulnerabilities, including the three we worked on. This feature, unique to the extreme ease of installation and use, led us to select Slither as a benchmark for our work.
\\\midrule[.3pt]
%
\parbox[t]{3em}{\ALIGN Smart\\ Check\\[.5ex]\cite{SmartCheck}}
	& Static checker via an XML-based intermediate representation. Vulnerabilities: 21 in total (see \cite{SmartCheck}).
	& \NOPE
	& Deprecated since 2020, failing for Solidity v0.6.0 and above, which reduces severely the test set of smart contracts.
%%	It runs lexical and syntactical analysis on Solidity source code. SmartCheck translates Solidity source code into an XML-based intermediate representation and checks it against XPath patterns. This tool covers 21 different types of vulnerabilities, including the three of interest to us. Unfortunately, however, the project is deprecated as of 2020, and it is stated by the authors that malfunctions may result on Solidity versions 0.6.0 and above. Given the limited applicability of the tool on the collected contracts, we decided not to use it as a benchmark.
\\\midrule[.3pt]
%
\TOOL{Remix}
	& Static checker (Remix Analysis is a plugin of Remix, the official \IDE of Solidity). Vulnerabilities: 7 types, including reentrancy, unchecked external call, and timestamp dependence.
	& \YEP
	& Most functional out-of-the-box tool found, offered via package managers and even via an online version. Vulnerabilities match our interest set.
%%	Remix Project is a rich toolset including Remix IDE, a comprehensive smart contract development tool. Within the IDE we can find the Solidity Analyzers plugin, which gangs three analysis tools together, including Remix Analysis, to perform static analysis on Solidity smart contracts. What led us to choose this tool, or rather this project, as a benchmark were the coverage of a wide type of vulnerabilities and the convenience of having an online version available, which can be used immediately and easily, without the need for installation on one's own machine.
\\\arrayrulecolor{black}\bottomrule
\end{tabular}

